IDA-VLM: Towards Movie Understanding via ID-Aware Large Vision-Language Model

The rapid advancement of Large Vision-Language models (LVLMs) has demonstrated a spectrum of emergent capabilities. Nevertheless, current models only focus on the visual content of a single scenario, while their ability to associate instances across different scenes has not yet been explored, which is essential for understanding complex visual content, such as movies with multiple characters and intricate plots. Towards movie understanding, a critical initial step for LVLMs is to unleash the potential of character identities memory and recognition across multiple visual scenarios. To achieve the goal, we propose visual instruction tuning with ID reference and develop an ID-Aware Large Vision-Language Model, IDA-VLM. Furthermore, our research introduces a novel benchmark MM-ID, to examine LVLMs on instance IDs memory and recognition across four dimensions: matching, location, question-answering, and captioning. Our findings highlight the limitations of existing LVLMs in recognizing and associating instance identities with ID reference. This paper paves the way for future artificial intelligence systems to possess multi-identity visual inputs, thereby facilitating the comprehension of complex visual narratives like movies.

==> sections/related_work.tex <==
\section{Related Work}

\subsection{Large Vision-Language Models}

Conventional multimodal models consist of uni-modal encoders and cross-modal fusion encoders. Relying on vision-language pre-training~\cite{DBLP:conf/emnlp/TanB19/lxmert, DBLP:conf/nips/LuBPL19/vilbert, Dou_2022_CVPR/meter, DBLP:conf/emnlp/WangJSYS21/mirtt, DBLP:conf/cvpr/JiWGZZWZSY23/map}, they have shown an impressive cross-modal semantic alignment ability~\cite{DBLP:conf/cvpr/JiTJKCZWY023/scl, DBLP:journals/corr/abs-2306-07096/glscl}, which brings substantial advances on various downstream tasks~\cite{balanced_vqa_v2/vqa_v2, DBLP:journals/ijcv/PlummerWCCHL17/f30k, DBLP:conf/eccv/LinMBHPRDZ14/mscoco}. However, due to the limitations of model size and training data scale, the performance of vision-language pre-training models is unsatisfied in open-ended scenarios.

Nowadays, Large language model (LLM) has exhibited remarkable abilities to understand, reason, and generate texts. Large Vision-Language Model (LVLM)~\cite{DBLP:journals/corr/abs-2311-12793/sharegpt4v, DBLP:conf/nips/Dai0LTZW0FH23/instructblip, DBLP:journals/corr/abs-2401-16420/intern} incorporates visual encoder and LLM, aligning visual features to the embedding space of LLM. Leveraging strong generalization and emergent capability of LLM, LVLM realizes free multimodal interactions with human. 
Flamingo~\cite{DBLP:conf/nips/AlayracDLMBHLMM22/flamingo} is a pioneering work on extending LLMs to vision-language pretraining by inserting additional cross-attention layers for visual input. 
BLIP-2~\cite{DBLP:conf/icml/0008LSH23/blip2} proposes Q-former to map the visual features to the hidden space of language models. 
To date, various works have shown encouraging progress with instruction tuning, including MiniGPT-4~\cite{DBLP:journals/corr/abs-2304-10592/minigpt4}, LLaVA~\cite{DBLP:conf/nips/LiuLWL23a/llava}, Otter~\cite{DBLP:journals/corr/abs-2305-03726/otter}, which demonstrate impressive results on natural instruction-following and visual reasoning capabilities. 
The perceptual capabilities of LVLMs are evolving towards fine-grained understanding. 
Numerous models~\cite{DBLP:journals/corr/abs-2307-03601/gpt4roi, DBLP:conf/nips/LiuLWL23a/llava, DBLP:journals/corr/abs-2306-15195/shikra, DBLP:conf/nips/WangCCWZZLLZQD23/visionllm} focus on region-level understanding, using visual instruction tuning with RoI reference, so that users could ask questions about specific instances within the content. 
Moreover, there are some LVLMs equiped with Stable Diffusion, which can produce multimodal outputs~\cite{DBLP:conf/nips/KohFS23/gill, DBLP:journals/corr/abs-2310-01218/seed,DBLP:journals/corr/abs-2307-05222/emu,DBLP:journals/corr/abs-2309-08637/textbind}. 
% The emergence and generalization capabilities displayed by LVLMs in open-ended scenarios have sparked endless imagination among people. 
LVLMs hold the potential to perform a wider array of functions and to understand more intricate visual information. 
For instance, movie is considered as one of the most intricate mediums for conveying visual information. 
% Movie understanding represents a considerable departure from conventional video understanding, which typically limits to a single scenario or activity. 
This paper researches on movie understanding with ID reference, recognizing characters across disparate scenes.

% For instance, they could comprehend an entire film or animation by recognizing and interpreting the roles and actions of characters.

% Current Large Vision Language Models (LVLMs) possess the capability to identify specific instances, such as recognizing celebrities within images. 
% The fine-grained features of individual instance are encapsulated as knowledge in the model's parameters during training. 
% In contrast, this paper focuses on the unique ability to memorize instance identities in real-time context and subsequently recognize them across different images.

\subsection{Multimodal Benchmark}
Previous evaluation for multimodal models measures some specific abilities, such as VQAv2~\cite{balanced_vqa_v2/vqa_v2}, GQA~\cite{DBLP:conf/cvpr/HudsonM19/gqa} for visual question answering, RefCOCO~\cite{DBLP:conf/emnlp/KazemzadehOMB14/refcoco} for visual grounding, Visual7W~\cite{DBLP:conf/cvpr/ZhuGBF16/v7w} for PointQA, VCR~\cite{DBLP:conf/cvpr/ZellersBFC19/vcr} for commonsense reasoning in an image. 
Recently, there is a surging interest in developing comprehensive benchmarks for evaluating LVLMs. 
MMBench~\cite{DBLP:journals/corr/abs-2307-06281/mmbench} consists of multiple-choice questions and introduces a CircularEval strategy for evaluation framework. 
LLaVA-Bench~\cite{DBLP:conf/nips/LiuLWL23a/llava} employs GPT-4 to assess responses from both GPT-4 and the model under evaluation, then provides scores and explanations for the answers. 
MM-Vet~\cite{DBLP:journals/corr/abs-2308-02490/mmvet} assesses LVLMs across six fundamental visual-linguistic capabilities, utilizing a GPT-4-based evaluator for open-ended responses. 
MME~\cite{DBLP:journals/corr/abs-2306-13394/mme} tests for perception and cognition competencies across 14 distinct subtasks, which requires models to provide simple `yes' or `no' answers. 
SEED-Bench~\cite{DBLP:journals/corr/abs-2307-16125/seedbench} covers 12 evaluation dimensions and adopts an answer ranking strategy to evaluate LVLMs via multiple-choice questions. 
POPE~\cite{DBLP:conf/emnlp/LiDZWZW23/pope} is a dedicated benchmark for assessing object hallucination. 
% prompting the model to ascertain whether specific objects appear in an image. 
% Benchmarks that use GPT-4 for evaluation typically feature a limited data scale, e.g., a mere 60 questions for LLaVA-Bench and 218 questions for MM-Vet. 
Existing benchmarks evaluate multifaceted performance of LVLMs, yet they predominantly focus on visual scenarios that lack character identities and intricate plots. 
 
% Compared to video understanding benchmark, 
